Modeling photoassociative spectra of ultracold NaK+K

A model for photoassociation of ultracold atoms and molecules is presented, and applied to the case of $^{39}$K and $^{23}$Na$^{39}$K bosonic particles. The model relies on the assumption that photoaossociation is dominated by long-range atom-molecule interactions, well outside the chemical bond region. The frequency of the photoassociation laser is chosen close to a bound-bound rovibronic transition from the $X^1\Sigma^+$ ground state toward the metastable $b^3\Pi$ lowest excited state of $^{23}$Na$^{39}$K, allowing to neglect any other excitation which could hinder the photoassociation detection. The energy level structure of the long-range $^{39}$K$\cdots$$^{23}$Na$^{39}$K excited super-dimer is computed in the space-fixed frame by solving coupled-channel equations, involving the coupling between the $^{23}$Na$^{39}$K internal rotation with the mechanical rotation of the super-dimer complex. A quite rich structure is obtained, and the corresponding photoassociation rates are presented. Other possible photossociation transitions are discussed in the context of the proposed model.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
      system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
